Assessing and marginalizing over compact binary coalescence waveform systematics with RIFT

As Einstein's equations for binary compact object inspiral have only been approximately or intermittently solved by analytic or numerical methods, the models used to infer parameters of gravitational wave (GW) sources are subject to waveform modeling uncertainty. Using a simple scenario, we illustrate these differences, then introduce a very efficient technique to marginalize over waveform uncertainties, relative to a pre-specified sequence of waveform models. Being based on RIFT, a very efficient parameter inference engine, our technique can directly account for any available models, including very accurate but computationally costly waveforms. Our evidence and likelihood-based method works robustly on a point-by-point basis, enabling accurate marginalization for models with strongly disjoint posteriors while simultaneously increasing the reusability and efficiency of our intermediate calculations.

==> future_work.tex <==

Parameter estimation of gravitational wave signals is a key part of GW astronomy and astrophysics. 
The inferred parameters are further utilized in the study for tests of GR, binary black hole population 
modeling, etc. Waveforms are computed . The current waveform models being used are both time-domain and frequency domain. Surrogate 
waveform models give more accurate results but are computationally expensive. 

\begin{itemize}

\item This project aims to assess the nature and impact of systematic differences between 
different waveform approximations for binary black hole, binary neutron star, and black hole/neutron 
star mergers~\cite{Ashton:2019leq}\cite{Veitch:2014wba}\cite{Purrer:2019jcp}.
\item Many waveform templates out there, need a study that compares them to look for biases(if they exist)
 and deduce if they are due to noise statistics/systematics or underlying physics(phenomenological models, 
 NR simulations, NRhybrid waveforms). For BBH we hope to get a better understanding of the usage of
 higher modes(sub-dominant) in waveforms~\cite{Shaik:2019dym}.
 \item Statistical differences will arise due to noise fluctuations in the received signal, whereas systematic 
 differences will arise due to the inherent difference in the models/underlying physics.
 \item Also look for effects of spins(zero, aligned, anti-aligned, precessing) of the compact binary on 
 parameter estimation(PE) of the GW signal.
 \item  \textbf{Goal: translate PP plot results to better identify accuracy standards.} Doing for many 
 events will help in population estimates.

\end{itemize}

